Efficient Single-Source Shortest Path and Distance Queries on Large Graphs

This paper investigates two types of graph queries: {\em single source distance (SSD)} queries and {\em single source shortest path (SSSP)} queries. Given a node $v$ in a graph $G$, an SSD query from $v$ asks for the distance from $v$ to any other node in $G$, while an SSSP query retrieves the shortest path from $v$ to any other node. These two types of queries are fundamental building blocks of numerous graph algorithms, and they find important applications in graph analysis, especially in the computation of graph measures. Most of the existing solutions for SSD and SSSP queries, however, require that the input graph fits in the main memory, which renders them inapplicable for the massive disk-resident graphs commonly used in web and social applications. The only exceptions are a few techniques that are designed to be I/O efficient, but they all focus on undirected and/or unweighted graphs, and they only offer sub-optimal query efficiency. To address the deficiency of existing work, this paper presents {\em Highways-on-Disk (HoD)}, a disk-based index that supports both SSD and SSSP queries on directed and weighted graphs. The key idea of HoD is to augment the input graph with a set of auxiliary edges, and exploit them during query processing to reduce I/O and computation costs. We experimentally evaluate HoD on both directed and undirected real-world graphs with up to billions of nodes and edges, and we demonstrate that HoD significantly outperforms alternative solutions in terms of query efficiency.

==> 4-SingleSource/singlesource.tex <==

\section{Algorithm for SSD Queries} \label{sec:sssp}

Given an SSD query from a node $s$ that is not in the core graph $\GC$, HoD processes the query in three steps:
\begin{enumerate}[itemsep = 0.5mm, topsep = 2mm]
\item {\bf Forward Search:} HoD traverses the forward graph $\GF$ starting from $s$, and for each node $v$ visited, computes the distance from $s$ to $v$ in $\GF$.

\item {\bf Core Search:} HoD reads the core graph $\GC$ into the main memory, and continues the forward search by following the outgoing edges of each node in $\GC$.

\item {\bf Backward Search:} HoD linearly scans the backward graph $\GB$ to derive the exact distance from $s$ to any node not in $\GC$.
\end{enumerate}
On the other hand, if $s$ is in $\GC$, then HoD would answer the query with a core search followed by a backward search, skipping the forward search. In what follows, we will present the details of three searches performed by HoD. For convenience, we define an {\em index} value $\theta(v)$ for each node {\em not} in the core graph $\GC$, such that $\theta(v) = i$ only if the $i$-th adjacency list in $\GF$ belongs to $v$. By the way $\GF$ is constructed (see Section~\ref{sec:pre-file}), for any two nodes $u$ and $v$ with $\theta(u) < \theta(v)$, the rank of $u$ is no larger than the rank of $v$.

\subsection{Forward Search} \label{sec:sssp-forward}

The forward search of HoD maintains a hash table $\HF$ and a min-heap $\QF$. In particular, $\HF$ maps each node $v$ to a key $\kf(v)$, which equals the length of the shortest path from $s$ to $v$ that is seen so far. Initially, $\kf(s) = 0$, and $\kf(v) = +\infty$ for any node $v \ne s$. On the other hand, each entry in $\QF$ corresponds to a node $v$, and the key of the entry equals $\theta(v)$, i.e., the index of $v$. As will become evident shortly, $\QF$ ensures that the forward search visits nodes in ascending order of their indices, and hence, it scans the file structure of $\GF$ only once, without the need to backtrack to any disk block that it has visited before.

HoD starts the forward search by inspecting each edge $e = \langle s, v\rangle$ adjacent to $s$ in $\GF$, and then inserting $v$ into $\HF$ with a key $\kappa(v) = l(e)$. (Note that $\GF$ contains only outgoing edges.) In addition, HoD also inserts $v$ into $\QF$. After that, HoD iteratively removes the top entry $u$ in $\QF$, and processes $u$ as follows: for each edge $e = \langle u, v\rangle$ adjacent to $u$, if $\kf(v) = +\infty$ in the hash table $\HF$, HoD sets $\kf(v) = \kf(u) + l(e)$ and inserts $v$ into $\QF$; otherwise, HoD sets $\kf(v) = \min\{\kf(v), \kf(u) + l(e)\}$. When $\QF$ becomes empty, HoD terminates the forward search, and retains the hash table $\HF$ for the second step of the algorithm, i.e., the core search.

%Given an SSD query from a source node $s$, HoD processes the query in three steps:
%\begin{enumerate}%[itemsep = 1mm, topsep = -1mm, partopsep = 0mm]
%\item {\bf Forward Search:} HoD traverses the forward graph $\GF$ and, for each node $v$ visited, computes the distance from $s$ to $v$ in $\GF$.
%
%\item {\bf Core Search:} HoD loads the core graph $\GC$ into the main memory, and computes the exact distance from $s$ to every node in $\GC$.
%
%\item {\bf Reversed Search:} HoD linearly scans the reverse graph $\GR$ to derive the exact distance from $s$ to any node not in $\GC$.
%\end{enumerate}
%In the following, we will present the details of each step.
%
%%For convenience, we use $v_i$ ($i \ge 1$) to denote the owner of the $i$-th adjacency list in $\GF$ (i.e., the adjacency list stores the outgoing edges of $v_i$). Note that for any node $v_j$ ($j > i$), its rank $r(v_j)$ must be no smaller than the rank $r(v_i)$ of $v_i$, as explained in Section~\ref{sec:pre-terminate}. In addition, in $\GR$, the adjacency list of $v_j$ is placed before that of $v_i$, since $\GR$ store adjacency list in the opposite order.
%
%\subsection{Forward Search} \label{sec:sssp-forward}
%
%The forward search of HoD maintains a hash table $H$ and a min-heap $Q^f$. In particular, $H$ maps each node $v$ to a key $\kappa(v)$, which equals the length of the shortest path from $s$ to $v$ that is seen so far. Initially, $\kappa(s) = 0$, and $\kappa(v) = +\infty$ for any node $v \ne s$. On the other hand, each entry in $Q^f$ corresponds to a node $v$, and the key of the entry equals {\em the position of $v$'s adjacency list in the forward graph $\GF$}. As will become evident shortly, $Q^f$ ensures that HoD can perform the forward search by scanning the file structure of $\GF$ once, without the need to backtrack to any disk block that it has visited before.
%
%In the beginning of the forward search, HoD inspects each edge $e = \langle s, v\rangle$ adjacent to $s$ in $\GF$, and then inserts $v$ into $H$ with a key $\kappa(v) = l(e)$. (Note that $\GF$ contains only outgoing edges.) In addition, HoD also inserts $v$ into $Q^f$.
%
%After that, HoD iteratively removes the top entry $u$ in $Q^f$, and processes $u$ as follows: for each edge $e = \langle u, v\rangle$ adjacent to $u$, if $\kappa(v) = +\infty$ in the hash table $H$, HoD sets $\kappa(v) = \kappa(u) + l(e)$ and inserts $v$ into $Q^f$; otherwise, if $\kappa(v) < +\infty$ and $\kappa(v) > \kappa(u) + l(e)$, HoD sets $\kappa(v) = \kappa(u) + l(e)$. When $Q^f$ becomes empty, the forward search terminates, and the hash table $H$ is handed over to the next step of the query algorithm, i.e., the core search.

\subsection{Core Search} \label{sec:sssp-core}

The core search of HoD is a continuation of the forward search, and it inherits the hash table $\HF$ created during the forward search. In addition to $\HF$, HoD creates a min-heap $\QC$, such that $\QC$ stores entries of the form $\langle v, \kf(v)\rangle$, where $v$ is a node and $\kf(v)$ is the key of $v$ in $\HF$. For any node $u$ with $\kf(u) \ne +\infty$ (i.e., $u$ is visited by the forward search), HoD inserts $u$ into $\QC$.

Given $\HF$ and $\QC$, HoD performs the core search in iterations. In each iteration, HoD extracts the top entry $v$ from $\QC$, and examines each outgoing edge $e$ of $v$. For every such edge, HoD inspects its ending point $w$, and sets $\kf(w) = \min\{\kf(w), \kf(v) + l(e)\}$. Then, HoD adds $w$ into $\QC$ if $w$ is currently not in $\QC$. This iterative procedure is repeated until $\QC$ becomes empty. After that, the hash table $\HF$ is sent to the last step (i.e., the backward search) for further processing.

\subsection{Backward Search} \label{sec:sssp-backward}

Given the hash table $\HF$ obtained from the core search, the reversed search of HoD is performed as a sequential scan of the backward graph $\GB$, which stores nodes in descending order of their index values. For each node $v$ visited during the sequential scan, HoD checks each edge $e = \langle u, v\rangle$ adjacent to $v$. (Note that $\GB$ contains only incoming edges). If $\kf(u) \ne +\infty$ and $\kf(u) + l(e) < \kf(v)$, then HoD sets $\kf(v) = \kf(u) + l(e)$. Once all nodes in $\GB$ are scanned, HoD terminates the backward search and, for each node $v$, returns $\kf(v)$ as the distance from $s$ to $v$.

One interesting fact about the backward search is that it does not require a heap to decide the order in which the nodes are visited. This leads to a much smaller CPU cost compared with Dijkstra's algorithm, as it avoids all expensive heap operations.

\subsection{Correctness and Complexities} \label{sec:sssp-proof}

Compared with Dijkstra's algorithm, the main difference of HoD's query algorithm is that it visits nodes in a pre-defined order based on their ranks. The correctness of this approach is ensured by the shortcuts constructed by the preprocessing algorithm of HoD. In particular, for any two nodes $s$ and $t$ in $G$, it can be proved that the augmented graph $\G$ always contains a path $P$ from $s$ to $t$, such that (i) $P$'s length equals the distance from $s$ to $t$ in $G$, and (ii) $P$ can be identified by HoD with a forward search from $s$, followed by a core search and a backward search. More formally, we have the following theorem.
\begin{theorem} \label{thrm:sssp-correct}
Given a source node $s$, the SSD query algorithm of HoD returns $\d(s, v)$ for each node $v \in G$.
\end{theorem}
Interested readers are referred to our online technical report \cite{HodReport} for the proof of Theorem~\ref{thrm:sssp-correct}.
%\begin{proof}
%Let $w$ be any node in $G$. By Lemma~\ref{lmm:p2p-correct}, HoD can correctly answer a PPD query from $s$ to $w$, which indicates that (i) there exists a path $P$ from $s$ to $w$ in the augmented graph, and (ii) $P$ can be identified by the combination of a forward search from $s$, a backward search from $w$, and a core search in $\GC$. Let $P_f$, $P_b$, and $P_c$ be the sub-paths of $P$ that is traversed by the forward, backward, and core searches of HoD, respectively.
%
%When processing the SSD query from $s$, HoD should be able to identify $P_f$, since the SSD query algorithm of HoD performs a forward search from $s$ that is exactly the same as in the PPD query algorithm. Meanwhile, since the semi-core search of HoD continues the forward search in $\GC$ using Dijkstra's algorithm, the path $P_c$ should also be found by HoD. Therefore, we can prove the lemma by showing that the reversed search of HoD can identify $P_b$.
%
%Without loss of generality, assume that $P_b = \langle v_1, v_2, \ldots, v_k, w\rangle$. Since $P_b$ is a path traversed by the backward search of HoD, we have $r(v_1) > r(v_2) > \ldots > r(v_k) > r(w)$. This indicates that the index values of $v_1, v_2, \ldots, v_k, w$ are in descending order, i.e., $\theta(v_1) > \theta(v_2) > \ldots > \theta(v_k) > \theta(w)$. Now recall that the reversed search of HoD (for any SSD query) is performed by a sequential scan of $\GB$, where nodes are stored in descending order of their index values. Therefore, the reversed search visits $v_i$ before $v_{i+1}$ ($i \in [1, k-1]$), and traverses $v_k$ before $w$. In other words, the path $P_b = \langle v_1, v_2, \ldots, v_k, w\rangle$ can be identified by the reversed search, which completes the proof.
%\end{proof}

%As with the case for PPD queries, HoD's algorithm for SSD queries requires $O(n + m_c)$ main memory. This is due to the fact that (i) the forward, semi-core, and reversed searches of HoD all maintain a hash table that takes $O(n)$ space, and (ii) the semi-core search requires reading the core graph $\GC$ into the memory. The time complexity of the algorithm is $O(n \log n + m')$, where $m'$ is the total number of edges in $\GC$, $\GF$, and $\GB$. The reason is that, when processing an SSD query, HoD may need to scan $\GF$, $\GC$, and $\GB$ once, and it may need to put $O(n)$ nodes into a min-heap. On the other hand, the I/O costs of the query algorithm is $O((n + m')/B)$, since it requires at most one scan of $\GF$, $\GC$, and $\GB$.


The query algorithm of HoD requires $O(n + m_c)$ main memory, where $m_c$ is the size of the core graph. This is due to the fact that (i) the forward, core, and back searches of HoD all maintain a hash table that takes $O(n)$ space, and (ii) the core search requires reading the core graph $\GC$ into the memory. The time complexity of the algorithm is $O(n \log n + m')$, where $m'$ is the total number of edges in $\GC$, $\GF$, and $\GB$. The reason is that, when processing an SSD query, HoD may need to scan $\GF$, $\GC$, and $\GB$ once, and it may need to put $O(n)$ nodes into a min-heap. Finally, the I/O costs of the algorithm is $O((n + m')/B)$, since it requires at most one scan of $\GF$, $\GC$, and $\GB$.



%\subsection{Optimization}

%This section presents {\em Arterial Hierarchy (AH)}, a scalable indexing method built upon the FC approach introduced in Section~\ref{sec:fc}. Compared with FC, AH has the same space complexity, a similar time complexity for distance queries, but significantly smaller pre-computation cost. In addition, AH also supports shortest path queries in a worst-case efficient manner.
%
%%In the following, we will XXXX
%
%\subsection{Overview} \label{sec:ah-overview}
%
%The main structure of AH is a node hierarchy $\H$ that resembles FC's node hierarchy $H$. In particular, both $\H$ and $H$ have $h+1$ levels, and both of their $i$-th levels ($i \in [0, h]$) is associated with a square grid $R_i$ of $2^{h+2 - i} \times 2^{h+2 - i}$ cells. However, AH and FC differ substantially in the ways that they decide node levels, construct shortcuts, and process queries.
%
%\header
%{\bf Differences in Node Levels.} To compute the level of each node, FC first imposes each $R_i$ on the road network $G$, and then computes the arterial edges in each ($4 {\times} 4$)-cell region in $R_i$, after which FC decides the node levels based on the arterial edges. As discussed in Section~\ref{sec:fc-complexity}, the derivation of arterial edges could incur significant overheads, since each ($4 {\times} 4$)-cell region in a coarse grid may cover a large number of nodes and edges in $G$.
%
%In contrast, AH computes node levels with an incremental algorithm that substantially improves efficiency. Given $G$, it first imposes the grid $R_1$ on $G$. Based on $R_1$, it identifies a set of unimportant nodes in $G$, and it assigns them to level $0$ of the node hierarchy $\H$. Then, it removes a subset of the unimportant nodes from $G$, and it constructs shortcuts between the remaining nodes. This results in a {\em reduced} graph $G_1$ that is considerably smaller than $G$. After that, AH recursively reduces $G_1$ into smaller graphs $G_2, G_3, \ldots G_h$, during which it assigns nodes to higher levels of $\H$. For the reduction from $G_{i}$ to $G_{i+1}$, AH needs to impose the grid $R_{i+1}$ on $G_{i}$ and compute the shortest paths in each ($4 {\times} 4$)-cell region. However, this computation is inexpensive since (i) $G_i$ has a much smaller size than $G$, and hence, (ii) each ($4 {\times} 4$)-cell region in $R_{i+1}$ contain only a small number of nodes or edges in $G_i$.
%
%\header
%{\bf Differences in Shortcuts.} FC creates only necessary shortcuts to ensure correct results for distance queries under the level and proximity constraints. In contrast, the shortcuts constructed by AH are not only for processing distance queries under the level and proximity constraints, but also for computing the actual shortest path between any two given nodes. Specifically, every shortcut $\langle v_a, v_c\rangle$ in AH's node hierarchy $\H$ is associated with a node $v_b$, such that (i) both $\langle v_a, v_b \rangle$ and $\langle v_b, v_c \rangle$ are edges in $\H$, and (ii) the length of $\langle v_a, v_c\rangle$ equals the lengths of $\langle v_a, v_b \rangle$ and $\langle v_b, v_c \rangle$ combined. In other words, $\langle v_a, v_c\rangle$ can be transformed into a two-hop shortest path $\langle v_a, v_b, v_c \rangle$. As such, given any path $P'$ in $\H$, we can transform $P'$ into a path in $G$, by recursively replacing each shortcut in $P'$ with its corresponding two-hop path.
%
%For example, Figure~\ref{fig:ah-recon} illustrates a shortest path $\langle v_1, v_2, \ldots, v_6\rangle$ in $G$, as well as three shortcuts $\langle v_1, v_4\rangle$, $\langle v_2, v_4 \rangle$, and $\langle v_4, v_6\rangle$. The shortcut $\langle v_1, v_4\rangle$ is associated with the node $v_2$, since $v_1$ is directly connected with $v_2$ and $v_2$ is directly connected with $v_4$. Similarly, $\langle v_2, v_4 \rangle$ and $\langle v_4, v_6\rangle$ are associated with $v_3$ and $v_5$, respectively. Now suppose that, given a distance query from $v_1$ to $v_6$, AH identifies $P' = \langle v_1, v_4, v_6\rangle$ as the shortest path from $v_1$ to $v_6$ in $\H$. To derive the actual shortest path from $v_1$ to $v_6$ in $G$, AH first replaces the shortcut $\langle v_1, v_4 \rangle$ in $P'$ with a two-hop path $\langle v_1, v_2, v_4 \rangle$, since $\langle v_1, v_4 \rangle$ is associated with $v_2$. This transforms $P'$ into another path $\langle v_1, v_2, v_4, v_6\rangle$. After that, we can replace $\langle v_2, v_4 \rangle$ with $\langle v_2, v_3, v_4 \rangle$, and substitute $\langle v_4, v_6\rangle$ with $\langle v_4, v_5, v_6\rangle$. As such, we obtain the shortest path $\langle v_1, v_2, \ldots, v_6\rangle$ from $v_1$ to $v_6$ in $G$.
%
%In general, given any shortest path query from a node $s$ to another node $t$, AH first computes the shortest path $P'$ from $s$ to $t$ in $\H$, and then it converts $P'$ into the corresponding path $P$ in the original road network. The conversion from $P'$ to $P$ takes only $O(k)$ time, where $k$ is the number of edges in $P$. This is because (i) for any shortcut in $\H$, we can identify its corresponding two-hop path in $O(1)$ time, and (ii) converting $P'$ to $P$ requires only $O(k)$ replacements of shortcuts.
%
%\header
%{\bf Differences in Query Processing.} Besides the aforementioned shortcuts (for reconstructing shortest paths), the node hierarchy $\H$ of AH also contains some extra shortcuts that can be leveraged for higher query efficiency. As a consequence, AH's query processing algorithm is slightly more sophisticated than FC's, as will be elaborated in Section~\ref{sec:ah-query}.
%
%\subsection{Index Construction} \label{sec:ah-pre}
%
%Similar to the case of FC, AH constructs its node hierarchy $\H$ in two steps: it first assigns each node in $G$ to a level in $\H$, and then it constructs shortcuts in $\H$ for query processing.
%
%%for all nodes in the same level, it orders the nodes based on a measurement of their relative importance. Finally, it creates shortcuts between nodes based on both the node levels and orderings.
%%
%\header
%{\bf Deciding Node Levels.}
%Given the road network $G$, AH first imposes on $G$ the grid $R_1$, where each cell contains at most one node. After that, AH identifies all ($4 {\times} 4$)-cell regions in $R_1$ that cover at least one node in $G$. For each of the ($4 {\times} 4$)-cell region identified, AH computes the arterial edges of the region in $O(1)$ time, and it marks each endpoint of an arterial edge as a {\em level-$1$ core}. At the same time, AH assigns all unmarked nodes to level $0$ of the node hierarchy $\H$ since, intuitively, those nodes are less important than the level-$1$ cores. After that, if any ($4 {\times} 4$)-cell region $B$ contains a local shortest path $P$ from a level-$1$ core $u$ to another level-$1$ core $v$, such that $P$ only goes through unmarked nodes, then AH inserts into $G$ a shortcut $\langle u, v\rangle$ with the same length as $P$. We say that $\langle u, v\rangle$ is a shortcut generated from $B$, and we use $G_1$ to denote the modified version of $G$ with all shortcuts added.
%%We also define the ID of $\langle u, v\rangle$ as the smallest ID of the edges on $P$.
%Overall, the computation of level-$1$ cores and the construction of $G_1$ takes only $O(n)$ time, since the number of non-empty ($4 {\times} 4$)-cell regions in $R_1$ is $O(n)$, and each of those regions contains $O(1)$ nodes and edges in $G$ (recall that $G$ is degree-bounded).
%
%For example, given the road network $G$ and the grid $R_1$ in Figure~\ref{fig:def-grid}, AH would identify $5$ level-$1$ cores: $v_7, v_8, v_9, v_{10}, v_{11}$. After adding shortcuts, $G$ is transformed into the graph $G_1$ in Figure~\ref{fig:ah-G0}. There exists a shortcut $\langle v_9$, $v_{10}\rangle$ in $G_0$ since (i) both $v_9$ and $v_{10}$ are level-$1$ cores, and (ii) in the ($4 {\times} 4$)-cell region $B$ illustrated in Figure~\ref{fig:def-grid}, the local shortest path between $v_9$ and $v_{10}$ goes only through $v_6$, which is unmarked. In general, the shortcuts in $G_1$ ensures that the level-$1$ cores form a connected graph even if we remove all unmarked nodes from $G_0$.
%
%%\header
%%{\bf Deciding Node Levels.}
%Given $G_1$, AH selects a subset of the level-$1$ cores in $G_1$ that are deemed more important than the others. The selected nodes are marked as the {\em level-$2$ cores}, while the remaining level-$1$ cores are assigned to level $1$ of $\H$. After that, AH converts $G_1$ into a smaller graph $G_2$ that retains all level-$2$ cores. This procedure is applied in a recursive manner: In the $i$-th recursion ($i \in [1, h-1]$), AH picks level-($i{+}1$) cores from the level-$i$ cores in $G_{i}$, and then it assigns the un-picked ones to level $i$ of $\H$, after which it transforms $G_{i}$ into a smaller graph $G_{i+1}$.
%
%A natural question is: Given $G_{i}$, how should AH select the level-($i{+}1$) cores from the level-$i$ cores? One straightforward solution is to construct a subgraph of $G_{i}$ that contains only the level-$i$ cores, and then compute the arterial edges in the subgraph to identify the more important nodes as level-($i{+}1$) cores. For example, given $G_1$ in Figure~\ref{fig:ah-G0}, we can first construct a subgraph of $G_1$ that contains only the five level-$1$ cores (i.e., $v_7, v_8, v_9, v_{10}, v_{11}$) and the edges connecting them (i.e., the five edges on the loop $\langle v_7, v_8, v_{10}, v_9, v_{11}, v_7\rangle$). After that, we impose the grid $R_2$ on the subgraph, compute the arterial edges, and then mark the endpoints of the arterial edges as level-$2$ cores. While this approach is intuitive, we find that (i) the resulting node hierarchy does not guarantee query correctness under the level and proximity constraints, and (ii) without the level and proximity constraints, it is difficult to achieve favorable asymptotic bounds on query time. To address this issue, we adopt a more careful approach to choose the level-($i{+}1$) cores without affecting the applicability of the level and proximity constraints in query processing. Specifically, our approach utilizes the concept of {\em border nodes}:
%\begin{definition}[Border Nodes] \label{def:ah-border}
%Let $B$ be a ($4 {\times} 4$)-cell region in $R_i$ ($i \in [1, h]$). A node $v$ in $G$ is a {\bf border node} of $B$, if (i) $v$ is not contained in the $2 \times 2$ cells centered at $B$, and (ii) $v$ is an endpoint of an edge in $G$ that intersects the boundary of the east, west, south, or north strip of $B$.
%\end{definition}
%
%\begin{figure}[t]
%%\begin{small}
%\begin{minipage}[t]{1.68 in}
%\centering
%%\hspace{3mm}
%\includegraphics[width = 1.64in]{./figures/PreAH6.eps}
%\figcapup \caption{Graph $G_1$.} \figcapdown \label{fig:ah-G0}
%\end{minipage}
%%\hspace{0.02in}
%\begin{minipage}[t]{1.68 in}
%\centering
%\includegraphics[width = 1.64in]{./figures/PreAH4.eps}
%%\vspace{-3.52mm}
%\figcapup \caption{Reduce graph $G'_1$.} \figcapdown \label{fig:ah-G0reduced}
%\end{minipage}
%%\end{small}
%\vspace{-2mm}
%\end{figure}
%
%For example, in Figure~\ref{fig:def-grid}, $v_1, v_2, v_9, v_{11}$ are all border nodes of the ($4 {\times} 4$)-cell region $B$, since each of them is an endpoint of an edge that intersects the boundary of $B$'s west strip, and none of them is contained in the $2\times2$ cells centered at $B$. Similarly, $v_3, v_4, v_7, v_8$ are also border nodes of $B$. On the other hand, $v_6$ and $v_{10}$ are not border nodes of $B$, since they are not adjacent to any edge that intersect the boundaries of $B$'s four strips.
%
%To select level-($i{+}1$) cores from $G_{i}$, we first reduce $G_{i}$ by removing any node in $G_{i}$ that is not a level-$i$ core and not a border node of any ($4 {\times} 4$)-cell region in $R_{i+1}$. We use $G'_{i}$ to denote the reduced graph thus obtained. For instance, given $G_1$ in Figure~\ref{fig:ah-G0}, we would remove $v_5$ and $v_6$, since none of them is a level-$1$ core or a border node in $R_2$. Figure~\ref{fig:ah-G0reduced} illustrates the reduced graph $G'_1$, with the border nodes in $R_2$ highlighted.
%
%Given $G'_{i}$, we impose $R_{i+1}$ on $G'_{i}$ and inspect each ($4 {\times} 4$)-cell region in $R_{i+1}$ that contains at least one node. For each such region $B$, we compute every spanning path of $B$ (see Definition~\ref{def:def-ae}) that satisfies two conditions:
%\begin{enumerate} [itemsep = 0.7mm, topsep = 1.5mm]
%\item {\em Border Condition:} The two endpoints of the path are border nodes of $B$, while the other nodes are all level-$i$ cores.
%
%\item {\em Coverage Condition:} Every shortcut on the path is generated from a region completely covered by $B$.
%\end{enumerate}
%For example, in the ($4 {\times} 4$)-cell region in Figure~\ref{fig:ah-G0reduced}, the spanning path $\langle v_2, v_9, v_{10}, v_8, v_3 \rangle$ satisfies both the border and coverage conditions, since (i) both $v_2$ and $v_3$ are border nodes, and (ii) the only shortcut on the path, $\langle v_9, v_{10} \rangle$, is generated from the region $B$ in Figure~\ref{fig:def-grid}, which is contained in the current ($4 {\times} 4$)-cell region.
%
%
%
%%We have the following lemma:
%%
%%\begin{lemma} \label{lmm:ah-pseudo}
%%Let $B$ be a ($4 {\times} 4$)-cell region in $R_i$ ($i \in [1, h]$), $P'$ be a path in $G'_{i-1}$, and $P$ be the path in $G$ that corresponds to $P'$. If $P'$ is a spanning path of $B$ that satisfies both the border and coverage conditions, then $P$ is a spanning path of $B$ in $G$.
%%\end{lemma}
%
%%By Lemma~\ref{lmm:ah-pseudo}, any spanning path $P$ in $G'_{i-1}$ that fulfills the border and coverage conditions can be mapped to a spanning path $P'$ in the original road network $G$. The correspondence between $P$ and $P'$ motivates us to identify important edges on $P$ in the same manner as on $P'$. In particular,
%
%For each spanning path $P$ that fulfills the border and coverage conditions, if it connects the west and east (resp.\ north and south) strips of $B$, we identify the edge\footnote{If multiple edges or shortcuts in $P$ intersect the bisector, we choose an arbitrary one among them as the pseudo-arterial edge.}
%%This does not affect the correctness or asymptotic bounds of AH.}
%in $P$ that intersects $B$'s vertical bisector (resp.\ horizontal bisector) as a {\em pseudo-arterial edge} of $B$. Observe that each pseudo-arterial edge of $B$ corresponds to a path in $G$ that contains an arterial edge of $B$. Intuitively, this indicates the importance of pseudo-arterial edges in the reduced graph $G'_{i}$. Accordingly, we mark the two endpoints every pseudo-arterial edge as level-($i{+}1$) cores, and we assign all unmarked level-$i$ cores to the $i$-th level of the node hierarchy $\H$. After that, for any local shortest path in a ($4 {\times} 4$)-cell region $B'$, if (i) the two endpoints of the path are either level-($i{+}1$) nodes or border nodes of $B'$, and (ii) other than its endpoints, the path does not go through any level-($i{+}1$) core, then we insert into $G'_{i}$ a shortcut between $u$ and $v$ with the same length as the local shortest path. Once all such shortcuts are added, we define the resulting graph as $G_{i+1}$, and we use it to recursively compute higher-level nodes in $\H$, as previously explained.
%
%It remains to show that we can efficiently derive the pseudo-arterial edges and construct shortcuts in $G'_{i}$. Let $B$ be a ($4 {\times} 4$)-cell region in $R_i$, and $u$ be a border node of $B$. Suppose that we invoke Dijkstra's algorithm to start a traversal of $G'_{i}$ from $u$; for each node visited, we follow the the outgoing edges of the node, ignoring any edge that violates the border condition or coverage condition. Once the traversal terminates, we can obtain the spanning paths of $B$ starting from $u$, as well as the pseudo-arterial edges on those edges. Similarly, with a traversal from $u$ that follows only the incoming edges of each node, we can compute the desired spanning paths of $B$ ending at $u$, along with the pseudo-arterial edges therein. By repeating this process on all border nodes of $B$, we can derive the set of all pseudo-arterial edges in $B$. With the same traversal algorithm, we can construct all shortcuts in $B$ using two traversals from each border node of $B$.
%
%%The aforementioned spanning paths can be easily computed with a slightly modified version of Dijkstra's algorithm. In particular, for each border node $u$ of $B$, we first apply Dijkstra's algorithm to perform a traversal starting from $u$. For each node $v$ that we visit, if $v$ is a level-($i{-}1$) core node, then we inspect any edge $\langle v, w\rangle$ going out form $v$, and we put $w$ into the priority queue if $w$ is contained in $B$. If $v$ is not a level-($i{-}1$) node, then $v$ must be a border node, if which case we omit all edges adjacent to $v$. Once the traversal terminates, we obtain all spanning paths starting from $u$ that satisfy both the border and coverage conditions. Similarly, we can also apply Dijkstra's algorithm to derive all spanning paths ending at $u$.
%%
%%converts $G_{i-1}$ into a smaller graph $G_i$ and assigns nodes to the $i$-th level of $\H$.
%%
%%would repeat a graph {\em reduction} procedure on $G_0$ for $h-1$ times, such that the $i$-th
%%
%%would focus on the core nodes in $G_0$, and then identify the
%%
%% such that the $i$-th step ($i \in [1, h-1]$) converts $G_{i-1}$ into a smaller graph $G_i$ and assigns nodes to the $i$-th level of $\H$. Specifically, to reduce $G_{i-1}$ to $G_i$, AH first removes from $G_{i-1}$ any edge connecting two non-core nodes. After that, it imposes the grid $R_i$ on $G_{i-1}$, and it eliminates any non-core node that is not a {\em border node} of any ($4 {\times} 4$)-cell region in $R_i$. The concept of border node is defined as follows:
%
%\header
%{\bf Creation of Shortcuts.} After the level of each node is decided, AH adds shortcuts in the node hierarchy $\H$ to facilitate query processing. The construction of shortcuts requires as input a strict total order on the nodes in the same level of $\H$. We will elaborate our ordering approach in Section~\ref{sec:ah-optimize}, but in general, any strict total order can be used without affecting the space and time complexities of AH. For our discussion that follows, it suffices to know that less important nodes tend to precede more important nodes in our strict total order. For convenience, we define a rank for each node in $G$, such that a node $u$ ranks lower than another node $v$, if (i) $v$ is at a higher level than $u$, or (ii) $u$ and $v$ have the same level, but $u$ precedes $v$ in the strict total order.
%
%AH constructs shortcuts in $\H$ in an incremental manner similar to the algorithm for deciding node levels. In particular, it first inspects $G$, and it inserts into $\H$ a set of shortcuts that are concern level-$0$ nodes. After that, it reduces $G$ to a smaller graph $\G_1$. Subsequently, it recursively reduces $\G_{i}$ into another graph $\G_{i+1}$ ($i \in [1, h-1]$), during which its constructs shortcuts that concern nodes at the $i$-th level of $\H$. In the following, we will elaborate the reduction from $\G_{i}$ to $\G_{i+1}$ ($i \in [0, h-1]$), assuming $\G_0 = G$. For convenience, we define the {\em level} of every edge in $\G_0$ as $-1$.
%
%Given $\G_{i}$, AH first imposes the grid $R_{i+1}$ on $\G_{i}$. For each node $u \in \G_i$, AH inspects the ($5 {\times} 5$)-cell region $C$ centered at $u$, as well as the subgraph of $\G_i$ that consists of any level-($i{-}1$) edge overlapping with $C$. Then, AH computes two {\em shortest path trees (SPT)} of the subgraph, as defined in the following:
%\begin{definition}[Shortest Path Trees (SPT)] \label{def:ah-spt}
%Let $G$ be a graph, and $T$ be a directed spanning tree of $G$ rooted at a node $u$. $T$ is a {\bf forward SPT} of $G$, if $T$ contains the shortest path from $u$ to any node in $G$. On the other hand, if $T$ contains the shortest path from any node in $G$ to $u$, then $T$ is a {\bf backward SPT} of $G$.
%\end{definition}
%
%Let $T_f$ (resp.\ $T_b$) be the forward (resp.\ backward) SPT of the aforementioned subgraph that is rooted at $u$. Observe that $T_f$ (resp.\ $T_b$) can be computed by one traversal of the subgraph using Dijkstra's algorithm. Let $v$ be any node in $T_f$, such that $u$ ranks lower than $v$ but higher than any ancestor of $v$ in $T_f$. For any such $v$, AH generates a shortcut $\langle u, v\rangle$ with a length equal to the distance from $u$ to $v$ in $T_f$. In addition, AH associates $\langle u, v\rangle$ with a node $w$ on the path from $u$ to $v$, such that $w$ ranks higher than any node on the path except $u$ and $v$. This is to indicate that, when answering shortest path queries, AH can replace $\langle u, v\rangle$ with a two-hop path $\langle u, w, v\rangle$. (Our algorithm guarantees that such a two-hop path always exists.) Similarly, for any node $v$ in $T_b$, AH creates a shortcut $\langle v, u\rangle$, if $u$'s rank is lower than $v$'s but higher than those of $v$'s ancestors in $T_b$. Furthermore, the shortcut is associated with the node $w'$ that ranks the highest among $v$'s ancestors except $u$.
%%For any node $v$ in the subgraph, let $P^+$ denote the path between $u$ and $v$ in $T^+$. If $v$ is the only node on $P^+$ that ranks higher than $u$, then AH adds a shortcut $\langle u, v\rangle$ into the node hierarchy $\H$, such that the length of $\langle u, v\rangle$ equals that of $P^+$.
%%
%%In addition, AH associates $\langle u, v\rangle$ with the node $w$ that immediately follows $u$ on $P^+$, i.e., $w$ is the neighbor of $u$ that lies on $P^+$.
%We refer to the shortcuts constructed above as {\em level-$i$ edges}\footnote{If multiple shortcuts are constructed from one node $u$ to another node $v$, AH retains only the shortest one.}. Intuitively, these shortcuts connect each level-$i$ node $u$ directly to its nearby higher-rank nodes. By following these shortcuts during query processing, AH can avoid visiting less important nodes, which helps improve efficiency.
%
%Besides the level-$i$ edges, AH creates a shortcut from $u$ and to a node $v$ in $T_f$ if (i) $u$ and $v$ are both at level $i$ or above, and (ii) all ancestors of $v$ except $u$ are below level $i$. Likewise, if $T_b$ contains a node $v$ with a level at least $i$, such that $u$ is the only ancestor of $v$ at level $i$ or higher, then AH generates a shortcut from $v$ to $u$. These shortcuts are to ensure that $\G_i$ would remain connected when we reduce $\G_i$ by removing some nodes below level $i$, as will be clarified shortly.
%
%When $i > 0$ (i.e., $\G_{i}$ is produced from a previous reduction step), AH also generates some extra shortcuts (referred to as {\em elevating edges}), in a manner slightly different from the construction of level-$i$ edges. First, AH inspects each node $u$ in $\G_{i}$ at a level lower than $i$, and it examines the ($5 {\times} 5$)-cell region $C$ in $R_{i+1}$ that is centered at $u$. Then, AH constructs a subgraph of $\G_{i}$ that comprises of all level-$i$ edges covered by $C$, {\em as well as all edges that connect $u$ with any node at level $i$ or above}. After that, AH computes the subgraph's forward and backward SPTs rooted at $u$. Let $P_f$ be any path in the forward SPT that connects $u$ to a node outside of $C$, and let $v$ the first node on $P_f$ at level $i$ or above (our algorithm ensures that such $v$ always exits). For every node $w$ preceding $v$ on $P_f$ (including $u$), we construct a shortcut $\langle w, v\rangle$, and we associate it with the node that immediately follows $w$ on $P_f$. The shortcut $\langle u, v\rangle$ is constructed to enable AH to efficiently traverse from $u$ to the $i$-th level of $\H$, while the other shortcuts $\langle w, v\rangle$ are generated to ensure that AH can map $\langle u, v\rangle$ to its corresponding path in $G$. Similarly, if the backward SPT contains a path $P_b$ that links $u$ with a node located beyond $C$, we identify the node $v$ that is closest to $u$ on $P_b$ among those nodes at level $i$ or above. For every node $w$ that precedes $v$ on $P_b$, we create a shortcut $\langle w, u\rangle$, and we associate it with the node that immediately precedes $w$ on $P_b$.
%
%
%
%%If the forward SPT contains a path $P_f$ from $u$ to a node $v$, such that $v$ is the only node on $P_f$ that ranks higher than $u$, then AH creates a shortcut $\langle u, v\rangle$ and associates it with the node that immediately succeeds $u$ on $P_f$. Similarly, for any path $P_b$ in the backward SPT that connects $u$ with a node $v$, if $u$ ranks higher than all other nodes on $P_b$ except $v$, then AH adds a shortcut $\langle v, u\rangle$ and associates it with the node the immediately follows $v$ on $P_b$. Intuitively, such elevating edges can help reduce query overhead, since they enable AH to traverse from lower-level nodes directly to higher-level nodes.
%
%%Let $P_f$ be a path in the forward SPT that connects $u$ to a node outside of $C$ (This occurs when the node is adjacent to an edge intersecting $C$'s boundary), and let $v$ be the first node on $P_f$ with a rank higher than $u$. For any such path $P_f$, we construct a shortcut $\langle w, v\rangle$ from every node $w$ preceding $v$ on $P_f$, and we associate the shortcut with the node that immediately follows $w$ on $P_f$.
%
%
%Once all level-$i$ edges and elevating edges are created, they are inserted into both $\G_i$ and $H$. After that, AH reduces $\G_i$ by retaining only (i) the border nodes in $R_{i+2}$ and (ii) nodes at level $i$ or above. The resulting graph is defined as $\G_{i+1}$ and is fed into the next reduction step.
%
%
%%It starts by imposing the grid $R_1$ on the road network $G$. For each node $u \in G$, AH inspects the ($5 {\times} 5$)-cell region $C$ centered at $u$, as well as the subgraph of $G$ that consists of any edge overlapping with $C$. Then, AH computes two {\em shortest path trees (SPT)} of the subgraph rooted at $u$, as defined in the following:
%%\begin{definition}[Shortest Path Trees (SPT)] \label{def:ah-spt}
%%Let $G$ be a graph, and $T$ be a directed spanning tree of $G$ rooted at a node $u$. $T$ is a {\bf forward SPT} of $G$, if $T$ contains the shortest path from $u$ to any node in $G$. On the other hand, if $T$ contains the shortest path from any node in $G$ to $u$, then $T$ is a {\bf backward SPT} of $G$.
%%\end{definition}
%%
%%Let $T^+$ (resp.\ $T^-$) be the forward (resp.\ backward) SPT of the aforementioned subgraph, such that both $T^+$ and $T^-$ are rooted at $u$. Observe that $T^+$ (resp.\ $T^-$) can be computed by one traversal of the subgraph starting from $u$, using the Dijkstra's algorithm. For any node $v$ in the subgraph, let $P^+$ denote the path between $u$ and $v$ in $T^+$. If $v$ is the only node on $P^+$ that ranks higher than $u$, then AH adds a shortcut $\langle u, v\rangle$ into the node hierarchy $\H$, such that the length of $\langle u, v\rangle$ equals that of $P^+$. In addition, AH associates $\langle u, v\rangle$ with the node $w$ that immediately follows $u$ on $P^+$, i.e., $w$ is the neighbor of $u$ that lies on $P^+$. This is to indicate that, when answering shortest path queries, AH may replace $\langle u, v\rangle$ with a two-hop path $\langle u, w, v\rangle$. (Our algorithm guarantees that the shortcut $\langle w, v\rangle$ would also be added into $\H$, when AH examines the ($5 {\times} 5$)-cell region centered at $w$.) Similarly, for any node $v$ in $T^-$, AH creates a shortcut $\langle v, u\rangle$ if, on the path from $v$ to $u$ in $T^-$, $v$ is the only node that ranks higher than $u$.
%
%\subsection{Node Ranking and Selection}\label{sec:ah-optimize}
%
%As mentioned, the shortcut construction algorithm of AH assumes that there is strict total order on the nodes in the same level. While any strict total order can be used without affecting the asymptotic bounds of AH, we have found a heuristic ordering approach that leads to high practical performance. Specifically, for nodes in the $0$-th level of the node hierarchy $\H$, we adopt a random order; for nodes in the $i$-th level ($i \in [1, h]$) of $\H$, we derive their ordering based on information from the preprocessing procedure of AH. To explain, recall that AH decides node levels by recursively applying a reduction procedure on the road network $G$. During the $i$-th reduction step ($i \in [1, h-1]$), AH examines a graph that contains level-($i{-}1$) cores; It identifies a set $S_i$ of pseudo-arterial edges in the graph, marks the endpoints of those edges as level-$i$ cores, and then assigns all unmarked level-($i{-}1$) cores to the ($i{-}1$)-th level of $\H$.
%
%We observe that the edges in $S_i$ are connected to some extend, and there are some level-$i$ cores that serve as hub nodes for the connections (i.e., they are adjacent to a relatively large number of edges in $S_i$). Intuitively, those hub nodes are more important than the rest of the level-$i$ cores. Motivated by this, we order the the level-$i$ cores using a {\em vertex cover} approach: we inspect the graph formed by the edges in $S_i$, and we compute a vertex cover of the graph using the standard linear-time $2$-approximation algorithm \cite{IntroAlgo}. The output of the algorithm is a sequence $\xi$ of nodes in the graph, such that the $i$-th node $v$ in $\xi$ is adjacent to the largest number of edges that are disjoint from the first $i-1$ nodes. Based on $\xi$, we order the level-$i$ cores as follows: The $i$-th node in $\xi$ is given the $i$-th highest rank, and the level-$i$ cores not in $\xi$ are given the lowest ranks arbitrarily.
%
%Interestingly, we find that if a level-$i$ core (i) does not appear in $\xi$ and (ii) is adjacent to a tiny number of edges in $\xi$, then we can downgrade it to a level-($i{-}1$) core without affecting correctness or asymptotic performance of AH. Such downgrading reduces the number of high-level nodes in the node hierarchy $\H$, which in turn improves query efficiency, since the high levels of $\H$ are frequently traversed during query processing. In our implementation of AH, we downgrade a level-$i$ core to level $i{-}1$ if it is absent from $\xi$ and is adjacent to less than $10$ edges in $S_i$.
%
%\subsection{Query Processing}\label{sec:ah-query}
%
%The query processing algorithm of AH is similar to that of FC. In particular, for distance query from a node $s$ to another node $t$, AH also answers the query with two traversals of the node hierarchy $\H$ starting from $s$ and $t$, respectively. As with the case of FC, each traversal of AH is performed with a constrained version of Dijkstra's algorithm. However, the constraints adopted by AH are slightly different: It adopts the proximity constraint (see Section~\ref{sec:fc-query}) and a {\em rank constraint} as follows:
%\begin{itemize}
%\item {\em Rank Constraint:} When the traversal from $s$ (resp.\ $t$) visits a node $u$, it ignores any neighbor of $u$ that ranks lower than $v$.
%\end{itemize}
%Intuitively, the rank constraint is a refined version of the level constraint, in that it takes into account not only the levels of nodes but also the strict total order defined on each level of $\H$. It leads to higher query efficiency as it helps AH bypass a larger number of relative unimportant nodes during query processing.
%
%In addition, AH also exploits the elevating edges in $\H$ (see Section~\ref{sec:ah-pre}) to reduce query cost, based on the following lemma:
%\begin{lemma} \label{lmm:ah-longpath}
%For any two nodes $u,v \in G$, if no ($4 {\times} 4$)-cell region in $R_i$ ($i \in [1, h]$) can cover $u$ and $v$ simultaneously, then the shortest path from $u$ to $v$ must go through a node at level $i$ or above.
%\end{lemma}
%Let $R_j$ ($j \in [1, h]$) be the coarsest grid where no ($4 {\times} 4$)-cell region contains both $s$ and $t$. By Lemma~\ref{lmm:ah-longpath}, the shortest path from $s$ to $t$ should pass through at least one node with a level at least $j$. This indicates that AH's traversal from $s$ would meet its traversal from $t$ at level $j$ or above. Therefore, if $s$ is a border node in $R_j$ (in which case $s$ has elevating edges to level $j$), then when we start the traversal from $s$, we can follow the elevating edges of $s$ to move directly to level $j$, ignoring any edge that connects $s$ to a node at a level lower than $j$. After that, we can continue the traversal from level $j$ under the rank and proximity constraints.
%
%More generally, for any level-$i$ ($i < j$) node $v$ visited in the traversal from $s$, if $v$ is a border node in $R_j$, then we move along the elevating edges of $v$ to level $j$ or above, omitting any other edges of $v$. On the other hand, if $v$ is a border node in $R_{j'}$ instead of $R_j$  ($j' < j$), then we follow the elevating edges $v$ to level $j'$ or higher, i.e., we traverse as close to level $j$ as possible. Meanwhile, if $v$ does not have any elevating edges or $v$ is at a level at least $j$, then we traverse the edges of $v$ that satisfies the rank and proximity constraints. The same strategy is used when AH traverses from $t$. This traversal strategy reduces query time, since it enables AH to avoid visiting the low levels of node hierarchy $\H$.
%
%So far we have only discussed distance queries. For any shortest path query from $s$ to $t$, AH first treats it as a distance query and computes the shortest path $P'$ from $s$ to $t$ in $\H$. After that, AH recursively replaces each shortcut in $P'$ with its corresponding two-hop path, which converts $P'$ to the actual shortest path from $s$ to $t$ in $G$, as explained in Section~\ref{sec:ah-overview}.
%
%\subsection{Space and Time Complexities}\label{sec:ah-complexity}
%
%To establish the space and time complexities of AH, we first introduce a lemma that quantifies the densities of nodes in each level of AH's node hierarchy $\H$:
%\begin{lemma} \label{lmm:ah-node-num}
%Any ($\alpha {\times} \alpha$)-cell region in $R_i$ contains $O(\alpha^2 \a^2)$ nodes whose level in $\H$ are no lower than $i$, where $\a$ is the arterial dimension of $G$.
%\end{lemma}
%Our proof of Lemma~\ref{lmm:ah-node-num} is similar to that of Lemma~\ref{lmm:fc-node-num}. We first show that any ($\alpha {\times} \alpha$)-cell region $B$ in $R_i$ contains the endpoints of $O(\alpha^2 \a)$ arterial edges in $G$. After that, we prove that there exists a one-to-many mapping from the arterial edges in $G$ to the nodes in $B$ with levels at least $i$, such that each edge is mapped to $O(\lambda)$ nodes. Based on this, we show that any ($\alpha {\times} \alpha$)-cell region in $R_i$ contains only $O(\alpha^2 \a^2)$ level-$i$ nodes of $\H$.
%
%\vspace{-0.3mm} \header
%{\bf Space Overhead.} Given Lemma~\ref{lmm:ah-node-num}, we can prove that each node in $\H$ has $O(h\a)$ elevating edges and $O(\a)$ non-elevating edges. This is because, by the preprocessing algorithm of AH, there is an elevating edge from a node $u$ to a level-$i$ node $v$, only if $u$ and $v$ are contained in the same ($4 {\times} 4$)-cell region in $R_i$. By Lemma~\ref{lmm:ah-node-num}, there exist $O(\a)$ such level-$i$ nodes. Since $\H$ contains only $h+1$ levels, that the total number of elevating edges adjacent to $u$ is $O(h\a)$. Similarly, we can prove that, when excluding elevating edges, each node in $\H$ has $O(\a)$ edges. Therefore, the space overhead of AH is $O(hn\a)$, which reduces to $O(hn)$ when $\a$ is a constant.
%
%\begin{table*}
%\centering
%\tblcapup \vspace{-1mm}
%\begin{small}
%\caption{Asymptotic performance of the state of the art.} \tblcapdown \vspace{-1mm}
%\label{tbl:related-complexity}
%\setlength{\extrarowheight}{0.1mm}
%%\begin{tabular}{|@{\hspace{1mm}}c@{\hspace{1mm}}|@{\hspace{1mm}}c@{\hspace{1mm}}|@{\hspace{1mm}}c@{\hspace{1mm}}|@{\hspace{1mm}}c@{\hspace{1mm}}|@{\hspace{1mm}}c@{\hspace{1mm}}|@{\hspace{1mm}}c@{\hspace{1mm}}|}
%%\begin{tabular}{|@{\hspace{1mm}}c@{\hspace{1mm}}|@{\hspace{1mm}}c@{\hspace{1mm}}|c|c|c|c|} \hline
%\begin{tabular}{|c|c|c|c|c|c|} \hline
%{\bf Reference} & {\bf  Space } &
%{\bf  Preprocessing} & {\bf Distance Query } & {\bf Shortest Path Query} & {\bf Remark}\\ \hline
%\multirow{2}{*}{\cite{ms12}} &  \gape[t]{$O(n)$} & $O(n \log n)$ & $O(n^{0.5+\epsilon})$ & N/A & \multirow{2}{5.4cm}{$S$ is a user-defined parameter in the range of $[n\log\log n, n^2]$. $D = l_{max}/l_{min}$, where $l_{max}$ (resp.\ $l_{min}$) is the largest (resp.\ smallest) road network distance between two nodes. $k$ is the number of edges in the shortest path between the source and destination of the query. $h$ is as defined in Section~\ref{sec:fc-pre}.}\\ \cline{2-5}
% & $O(S)$ & \gape[t]{$\tilde{O}(S)$} & $\tilde{O}(n/\sqrt{S})$ & N/A & \\ \cline{1-5}
%\multirow{2}{*}{\cite{afg10}} &  \gape[t]{$O(n \log n \log D)$} & $O(n^2 \log n)$ & $O(\log^2 n \log^2 D)$ & $O(k + \log^2 n \log^2 D)$ & \\ \cline{2-5}
% & \gape[t]{$O(n \log n \log D)$} & $O(n^2 \log n)$ & $O(\log n \log D)$ & N/A & \\ \cline{1-5}
%\cite{ssa08} &  $O(n\sqrt{n})$ & $O(n^2 \log n)$ & \gape[t]{$O(k\log n)$} & $O(k\log n)$ & \\ \cline{1-5}
%this paper &  $O(hn)$ & $O(hn^2)$ & \gape[t]{$O(h \log h)$} & $O(k + h\log h)$ &  \\ \hline
%%\cite{ssa09}  & road networks & $O(n)$ & $O(n^2 \log n)$ & $O(\log n \log D)$ & N/A \\ \cline{3-6}
%\end{tabular}
%\end{small}
%\tbldown \vspace{-1mm}
%\end{table*}
%
%\vspace{-0.3mm} \header
%{\bf Query Time.} AH answers any distance query with two traversals of $\H$, starting from the source $s$ and destination $t$ of the query, respectively. Due to the proximity constraint, in the $i$-th level of $\H$ ($i \in [0, h]$), each traversal of AH only visits the nodes in a ($5 {\times} 5$)-cell region in $R_{i+1}$. By Lemma~\ref{lmm:ah-node-num}, such a region only contains $O(\a^2)$ nodes at level $i$. Hence, the totally number of nodes traversed by AH is $O(h \a^2)$. Furthermore, for each node $v$ visited during a traversal, AH either follows the elevating edges of $v$ to a certain level of $\H$, or moves along the non-elevating edges of $v$ that satisfy the rank and proximity constraints. As previously discussed, $v$ has $O(\a)$ elevating edges to each level of $\H$, and has $O(\a)$ non-elevating edges. Therefore, the total number of edges visited by AH is $O(h \a^3)$. Since each traversal is performed using Dijkstra's algorithm, its overall time complexity is $O(h\a^2 \log(h\a^2) + h\a^3)$. Consequently, when $\a$ is a constant, the time complexity of AH for a distance query is $O(h \log h)$.
%
%To answer a shortest path query from $s$ to $t$, AH first processes its corresponding distance query to retrieve the shortest path $P'$ from $s$ to $t$ in $\H$, and then its transforms $P'$ into the actual shortest path $P$ from $s$ to $t$ in $G$. The transformation from $P'$ to $P$ takes $O(k)$ time, where $k$ is the number of edges in $P$. Therefore, AH requires $O(k + h \log h)$ time to answer a shortest path query.
%
%\header
%{\bf Preprocessing Cost.} The preprocessing algorithm of AH consists of three steps: (i) assigning nodes to each level of $\H$, (ii) deriving the strict total order on nodes at the same level, and (iii) creating shortcuts in $\H$. When assigning nodes to the $i$-th level of $\H$ ($i \in [0, h-1]$), AH inspects each non-empty ($4 {\times} 4$)-cell region in $R_{i+1}$, and construct a subgraph that consists of the level-$i$ cores and border nodes in the region. For each node in the subgraph, AH needs to apply Dijkstra's algorithm to traverse the subgraph a constant number of times. Given Lemma~\ref{lmm:ah-node-num} and the fact that each level-$i$ core or border node (i) has $O(\lambda^2)$ edges and (ii) is contained in a constant number of ($4 {\times} 4$)-cell region in $R_{i+1}$, it can be proved that AH require $O(n^2 \lambda^2)$ time to assign nodes to level $i$ of $\H$. Meanwhile, AH takes only $O(n)$ time to derive the strict total order at level $i$ of $\H$, since the derivation is based on a linear time algorithm for vertex cover.
%
%To construct shortcuts at the $i$-th level of $\H$, AH needs to inspect a graph $G^*_i$ reduced from $G$. For each node $u$ in $G^*_i$, AH examines the a ($5 {\times} 5$)-cell region in $R_{i+1}$ that is centered at $u$, and it creates shortcuts for $u$ by traversing the nodes in the region at level $i$ or above. Based on Lemma~\ref{lmm:ah-node-num}, it can be proved that total cost of generating shortcuts for $u$ is $O(\a^2)$. As such, the time required to create shortcut at level $i$ of $\H$ is $O(n \a^2)$.
%
%Summing up the above analysis, we have the following theorem:
%\begin{theorem} \label{thrm:ah-complexity}
%Given a road network with a constant arterial dimension, AH takes $O(h n^2)$ time to construct an index that requires $O(h n)$ space. With the index, AH answers any distance query in $(h \log h)$ time and any shortest path query in $O(k + h \log h)$ time, where $k$ is the number of edges in the shortest path.
%\end{theorem}
%
%%\section{Algorithm details}\label{sec:details}
%%This section covers two parts: (i) How to partition the nodes into levels and (ii) how to add shortcuts to the graph and further how the query works. For clarity in the following we describe the method on undirected graphs, and we will further modify the method to directed graphs in section \ref{subsec:directedgraphs}.
%%
%%\subsection{Layer Construction}\label{subsec:levelconstruct}
%%In this section we focus on the details of computing transit nodes at a certain iteration. Suppose we have already computed $V_0, V_1, \ldots, V_{i-1}$, now we are at the \textbf{$i$th} iteration and intend to compute $V_i$.
%%
%%\begin{algorithm}
%%\caption{$Compute\_Level(i, V_{i-1}, G=(V, E\cup E_{i-1}))$}\label{alg:main}
%%\begin{algorithmic}[1]
%%\State Impose a grid on $G$, the size of a cell is $g_i\times g_i$
%%\State $\mathcal{P} \leftarrow \varnothing$
%%\ForAll {cell $C$}
%%\ForAll {$s\in I_C$}
%%\State $G'\leftarrow SubGraph(C,E_{i-1})$
%%\State $T_s\leftarrow BuildDijkstraTree(s,G')$
%%\ForAll {$t\in O_C$}
%%\State $p\leftarrow FindLocalShortestPath(s,t,T_s)$
%%\State $\mathcal{P} \leftarrow \mathcal{P} \bigcup \{ p\}$
%%\EndFor
%%\EndFor
%%\EndFor
%%\State $V_i \leftarrow SelectTransitNode(\mathcal{P},i)$
%%\State $E_i \leftarrow AddShortcuts(V_i)$
%%\State return $V_i, E_i$
%%\end{algorithmic}
%%\end{algorithm}
%%
%%Algorithm \ref{alg:main} presents the computation process. $Compute\_Level$ has three input parameters. $i$ and $V_{i-1}$ are as described before. $E_{i-1}$ is a set of edges (original edges and generated shortcuts) computed at the ${i-1}$th iteration. The edges in $E_{i-1}$ are used to accelerate the local shortest path search in the current iteration. At the first iteration $E_0=E$. $Compute\_Level$ works in the following way: for each cell $C$, find out the local shortest path from an inner border node to an outer border node in the sub-graph centred at $C$. After the path is found, we can select the transit nodes by examining every shortest path, from which the endpoint of an edge that intersects the inner shell of $C$ is picked out. This selection could be done at between line 11 and line 12. Here we do a lazy-selection for optimization purpose, i.e. we select all the transit nodes after $\mathcal{P}$, the set of all the local shortest paths are obtained (line 13). In addition, to avoid redundant computation, we use a Dijkstra spanning tree to preserve the shortest paths information. Firstly we construct a Dijkstra spanning tree from an inner border node $s$ (line 6), then the shortest paths from $s$ to the outer border nodes could be quickly computed from that tree(line 8). After all the local shortest paths are computed, $SelectTransitNode$ selects the transit nodes $V_i$ (line 13), and subsequently we generate some shortcuts (line 14) and compute a set of edges $E_i$ in order to accelerate the local shortest paths search in the next iteration. Finally $V_i$ and $E_i$ are returned which serve as the input for the ${i+1}$th iteration.
%%
%%In the following we first describe how to add shortcuts, and then $BuildDijkstraTree$, $FindLocalShortestPath$ and $SelectTransitNode$ because the latter procedures use the shortcuts $E_i$ generated in the last iteration.
%%
%%\input{4-Algorithm_Details/adding_shortcuts.tex}
%%
%%\subsubsection{Finding local shortest path} \label{subsec:findshortestpath}
%%Now we focus on the local shortest path search of a cell $C$ (line 3 to line 9 in Algorithm ~\ref{alg:main}). A the beginning we impose a grid on the graph, then we compute the local shortest paths for each cell. As for a cell $C$, with the help of $E_{i-1}$, we can only consider the sub-graph composed of the edges in $E_{i-1}$ which overlap the outer shell of $C$. The first type of edges in $E_{i-1}$ guarantees that the inner border nodes (resp. outer border nodes) are connected with the nodes in $V_{i-1}$, and the second type of edges in $E_{i-1}$ guarantees the connectivity among the nodes in $V_{i-1}$. Then we run $BuildDijkstraTree$ to build a Dijkstra spanning tree $T_s$ rooted from an inner border node by traversing the sub-graph. In $FindLocalShortestPath$ we match the outer border node $t$ and the leaves of $T_s$ to form a local shortest path. Consider the example in Figure ~\ref{fig:level2}, we are about to compute the shortest path from the inner border node $v_2$. The sub-graph considered is the one $G'=(V',E')$ where $V'=\{v_1,v_2,v_3,v_4,v_7,v_8,v_9,v_{10},v_{11}\}$ and $E'=\{(v_2,v_9),(v_9,v_{11}),(v_1,v_{11}),(v_9,v_{10}),(v_{10},v_8),(v_8,v_7),(v_{11},v_7),(v_7,v_4),(v_3,v_8)\}$. At first we build a Dijkstra tree as shown in Figure ~\ref{fig:DijkstraTree}. Then we match $v_3$ and the leaves of the tree $v_7$, $v_8$ to form the local shortest path. Finally the local shortest path $(v_2,v_9,v_{10},v_8,v_3)$ is found.
%%
%%%\begin{figure}
%%%\centering
%%%\includegraphics[width = 3in]{figures/DijkstraTree.eps}
%%%\caption{Dijjkstra tree} \label{fig:DijkstraTree}
%%%\end{figure}
%%
%%\input{4-Algorithm_Details/select_transit_nodes.tex}
%%
%%\subsection{Query indexing and queries}\label{subsec:query}
%%After the preprocessing above, we have tagged each node with its highest layer flag. Then we partition the nodes into $h$ levels, with $h$ the height of the hierarchy: for $0\le i\le h$, $L_i$ is the set of nodes tagged with an layer $i$ flag. Consistent with the preprocessing, the nodes in $L_i$ are more important than the ones in $L_{i-1}$. Then we get an total order on $V$: each node is associated with a rank. The nodes in $L_{i+1}$ have a higher rank than those in $L_i$. As for the ones in the same level, say $L_i$, we rank them according to the number of paths in $\mathcal{P}$ they cover, i.e. the more local shortest paths in $\mathcal{P}$ a node covers, the higher the rank. We use $Rank_v$ to represent the rank associated to $v$.
%%
%%%\begin{figure}
%%%\centering
%%%\includegraphics[width = 3in]{figures/CH.eps}
%%%\caption{Contraction Order} \label{fig:CH}
%%%\end{figure}
%%
%%Now we remove all the shortcuts added before and rebuild the query index in the following way: we in turn contract the nodes in increasing order of their ranks. When contracting a node, say $v$, we remove $v$ after adding some shortcuts, which are called "\emph{query shortcuts}". For all pairs $u,w$ such that $u$ and $w$ are both adjacent to $v$, and both of them have higher ranks than $v$, we add a shortcut $(u,w)$ weighted $weight((u,v))+weight((v,w))$ if and only if the shortest path connecting $u$ and $w$ is the $(u,v,w)$ one. As shown in Figure ~\ref{fig:CH}, the numbering of the nodes is consistent with their ranks. The algorithm in turns contracts $v_1$ to $v_{11}$. when contracting $v_5$, its adjacent nodes are $v_8$ and $v_9$. Since the shortest path between $v_8$ and $v_9$ is not the $(v_8,v_5,v_9)$ one, so we do not add a shortcut. When contracting $v_6$, since the shortest path between $v_9$ and $v_{10}$ is the $(v_9,v_6,v_{10})$ one, so we add a shortcut $(v_9,v_{10})$. Similarly we add $(v_{10},v_{11})$ when contracting $v_9$. At a first glance the shortcuts may increase the data volume of $G$ which further slow down the queries, however, as we will see later, actually the shortcuts efficiently speed up the queries.
%%
%%With the shortcuts we can execute the query using a bidirectional Dijkstra method with some modifications. For a given source $s$ and a target $t$, we instantiate two Dijkstra searches respectively starting from $s$ and $t$. When $v$ is extracted from the priority queue, the algorithm only visit those nodes $u$ such that $u$ is adjacent to $v$ (by original edges or added shortcuts) and $Rank_u>Rank_v$. As shown in Figure ~\ref{fig:CH}, when we query the shortest path from $v_1$ to $v_3$, we instantiate two instances of Dijkstra traversal respectively from $v_1$ and $v_3$. Then we can reach $v_{11}$ and $v_8$. The search stalks at $v_{11}$ since none of the adjacent nodes of $v_{11}$ has a higher rank. When expanding $v_8$ it relaxes the edge $(v_8,v_{11})$ and $(v_8,v_{10})$. Finally the shortest path is found.  With the $Rank_u>Rank_v$ condition, the query does not need to visit all the nodes adjacent to $v$, which can reduce a large amount of unnecessary visits. Because, as the search continues, the number of adjacent nodes with higher ranks is limited. The query method can be proven correct. Due to space limit we omit the proof here.
%%
%%The query indexing and query method is similar to the \emph{Contraction Hierarchy(CH)}, but our method can be proven bounded in both space complexity and query time complexity due to the construction of the node ordering. As a contrast, the node ordering in \emph{CH} is constructed by heuristic methods which result in unstable complexities in both space and time.
%%
%%\subsection{proof of complexity} \label{subsec:proof}
%%(1) space complexity
%%(2) time complexity


==> 5-P2P/p2p.tex <==
\section{Algorithm for PPD Queries} \label{sec:p2p}

Suppose that we are given a PPD query from a source node $s$ to a destination node $t$. If both $s$ and $t$ are in the core graph $\GC$, then HoD first reads $\GC$ into the main memory, and then answers the query using an in-memory algorithm. On the other hand, if $s$ or $t$ is not in $\GC$, then the algorithm for processing the query is more sophisticated. In particular, in the most challenging case when neither $s$ nor $t$ is in $\GC$, HoD processes the query in three steps:
\begin{enumerate}%[itemsep = 1mm, topsep = -1mm, partopsep = 0mm]
\item {\bf Forward Search:} HoD traverses the forward graph $\GF$ starting from $s$, and for each node $v$ visited, computes the distance from $s$ to $v$ in $\GF$.

\item {\bf Backward Search:} This step is similar to the forward search, except that the graph being traversed is $\GB$, and the starting point of the traversal is $t$.

\item {\bf Core Search:} Given the distance information obtained in the first two steps, HoD loads the core graph $\GC$ into the main memory, and then derives the distance from $s$ to $t$.
\end{enumerate}
In what follows, we first present the details of each step for the case when $s$ and $t$ are not in $\GC$, and then we explain how the other cases can be handled. For convenience, we define an {\em index} value $\theta(v)$ for each node {\em not} in the core graph $\GC$, such that $\theta(v) = i$ only if the $i$-th adjacency list in $\GF$ belongs to $v$. By the way $\GF$ is constructed (see Section~\ref{sec:pre-terminate}), for any two nodes $u$ and $v$ with $\theta(u) < \theta(v)$, the rank of $u$ is no larger than the rank of $v$.

%use $v_i$ ($i \ge 1$) to denote the owner of the $i$-th adjacency list in $\GF$ (i.e., the adjacency list stores the outgoing edges of $v_i$). Note that for any node $v_j$ ($j > i$), its rank $r(v_j)$ must be no smaller than the rank $r(v_i)$ of $v_i$, as explained in Section~\ref{sec:pre-terminate}. In addition, in $\GR$, the adjacency list of $v_j$ is placed before that of $v_i$, since $\GR$ store adjacency list in the opposite order.

\subsection{Forward Search} \label{sec:p2p-forward}

The forward search of HoD maintains a hash table $\HF$ and a min-heap $\QF$. In particular, $\HF$ maps each node $v$ to a key $\kf(v)$, which equals the length of the shortest path from $s$ to $v$ that is seen so far. Initially, $\kf(s) = 0$, and $\kf(v) = +\infty$ for any node $v \ne s$. On the other hand, each entry in $\QF$ corresponds to a node $v$, and the key of the entry equals $\theta(v)$, i.e., the index of $v$. As will become evident shortly, $\QF$ ensures that the forward search visits nodes in ascending order of their indices, and hence, it scans the file structure of $\GF$ only once, without the need to backtrack to any disk block that it has visited before.

HoD starts the forward search by inspecting each edge $e = \langle s, v\rangle$ adjacent to $s$ in $\GF$, and then inserting $v$ into $\HF$ with a key $\kappa(v) = l(e)$. (Note that $\GF$ contains only outgoing edges.) In addition, HoD also inserts $v$ into $\QF$. After that, HoD iteratively removes the top entry $u$ in $\QF$, and processes $u$ as follows: for each edge $e = \langle u, v\rangle$ adjacent to $u$, if $\kf(v) = +\infty$ in the hash table $\HF$, HoD sets $\kf(v) = \kf(u) + l(e)$ and inserts $v$ into $\QF$; otherwise, if HoD sets $\kf(v) = \min\{\kf(v), \kf(u) + l(e)\}$. When $\QF$ becomes empty, HoD terminates the forward search, and retains the hash table $\HF$ for the third step of the algorithm, i.e., the core search.

\subsection{Backward Search} \label{sec:p2p-backward}

The backward search of HoD works in a manner very similar to the forward search, and it also maintains a hash table $\HB$ and a min-heap $\QB$. $\HB$ maps each node $v$ to a key $\kb(v)$, while $\QB$ sorts nodes according to their index values.

When the backward search starts, HoD sets $\kb(t) = 0$ and $\kb(v) = +\infty$ for any $v \ne t$, after which it inserts $t$ into $\QB$. Then, HoD iteratively extracts the top entry $u$ in $\QB$, and processes $u$ as follows. First, HoD examines the neighbors of $u$ in $\GB$ (recall that $\GB$ only records the incoming edges of each node). For each neighbor $v$, if $\kb(v) = +\infty$ in $\HB$, then HoD adds $v$ into $\QB$, setting $\kb(v)$ to the length of the edge $\langle u, v \rangle$; otherwise, if $\kb(v) > \kb(u) + l(\langle u, v \rangle)$, then HoD updates $\kb(v)$ to $\kb(u) + l(\langle u, v \rangle)$. The backward search completes when $\QB$ is empty, upon which HoD retrieves the hash table $\HB$ and moves on to the core search.

\subsection{Core Search} \label{sec:p2p-core}

The core search of HoD performs two traversals of the core graph $\GC$, and the first (resp.\ second) traversal is essentially a continuation of the forward (resp.\ backward) search. In particular, the core search uses the hash tables $\HF$ and $\HB$ created during the forward and backward searches, along with two new min-heaps $\QFF$ and $\QBB$. Each entry in $\QFF$ (resp.\ $\QBB$) corresponds to a node $v$, and the key of the entry equals the value $\kf(v)$ in $\HF$ (resp.\ $\kb(v)$ in $\HB$). This contrasts the forward and backward searches, which uses min-heaps where the key of each entry is the index value of a node. In addition, HoD also maintains a variable $\dm$ that records the smallest distance from $s$ to $t$ in the part of the augmented graph that has been traversed. Initially, $\dm = \min_v \big\{\kf(v) + \kb(v)\big\}$. (Observe that $\kf(v)$ is an upper-bound of the distance from $s$ to $v$ and $\kb(v)$ is an upper-bound of the distance from $v$ to $t$.)

As the first step of the core search, HoD inserts into $\QFF$ any node $u \in \GC$ with $\kf(u) \ne +\infty$ (i.e., $u$ is reached by the forward search previously). Similarly, it also adds into $\QBB$ any node $w \in \GC$ with $\kb(u) \ne +\infty$. After that, HoD removes the top entries from $\QFF$ and $\QBB$ in a round-robin fashion. Whenever it extracts an entry $u$ from $\QFF$, it inspects both $\kf(u)$ and $\kb(u)$. If $\kf(u) + \kb(u) < \dm$, then HoD sets $\dm = \kf(u)+\kb(u)$. In addition, for each outgoing edge $e = \langle u, v\rangle$ from $u$, HoD sets $\kf(v) = \min\{\kf(v), \kf(u) + l(e)\}$, and inserts $v$ into $\QFF$ (if $v$ has not been inserted before).

The core search terminates when $\dm$ is smaller than or equal to $\kf(u) + \kb(w)$, where $u$ and $w$ are the top entries in $\QFF$ and $\QBB$, respectively. The rationale is that, for any unseen entry $v$, the distance from $s$ to $v$ is at least $\kf(u)$, and the distance from $v$ to $t$ is at least $\kb(w)$. As a consequence, if $\dm \le \kf(u) + \kb(w)$, then the path from $s$ to $t$ via $v$ cannot be shorter than $\dm$. Upon termination of the core search, HoD returns $\dm$ as the result of the PPD query from $s$ to $t$.

\subsection{Degenerated Cases and Correctness} \label{sec:p2p-proof}

The above discussion assumes that neither $s$ or $t$ is in the core graph $\GC$. Nevertheless, HoD can easily handle the case when $s$ or $t$ is in $\GC$. In particular, if $s$ is in $\GC$, then HoD simply omits the forward search. Accordingly, the core search will use a hash table $\HF$ where $\kf(s) = 0$ and $\kf(v) = +\infty$ for every $v \ne s$. The case when $t$ is not in $\GC$ is handled similarly.

The following lemma shows the correctness of HoD's query algorithm for PPD queries:
\begin{lemma} \label{lmm:p2p-correct}
Given any source node $s$ and any destination node $t$, HoD correctly computes the distance from $s$ to $t$.
\end{lemma}
%\vspace{0mm}
\begin{proof}[Sketch]
Let $v_i$ ($i \ge 1$) be the node in $G_f$ with the $i$-th largest index value. We define $S_0$ as the set of nodes in $\GC$, and $S_i$ ($i \ge 1$) as a set that contains all nodes in $\GC$ as well as $v_1, v_2, \ldots, v_i$. We will use an induction on $i$ to show that, for any $S_i$, HoD can correctly compute the distance between any two nodes in $S_i$.

Consider the base case when $i = 0$. When both $s$ and $t$ are in $S_0$, HoD computes the distance from $s$ to $t$ based only on the nodes and edges in $\GC$. Recall that, in the preprocessing procedure of HoD, whenever we remove a node from the reduced graph, we always construct shortcuts between the remaining nodes, to ensure that the distance between any two remaining nodes is not affected. Therefore, the distance from $s$ to $t$ in $\GC$ should be equal to $\d(s, t)$, i.e., HoD should return correct result for the PPD query.

Assume that HoD can correctly compute the distance between any two nodes in $S_i$ ($i \ge 0$). Let $u$ be the node in $S_{i+1}$ but not $S_i$. We will first prove that HoD can correctly derive the distance from $u$ to any other node $v$ in $S_{i+1}$. First, since $v \in S_{i+1}$ and $v \ne u$, $v$ must be in $S_i$. Let $P$ be the shortest path from $u$ to $v$ in the original graph. Among the nodes in $S_i$ that also appear on $P$, let $w$ be the one that minimizes $\d(u, w)$. By the preprocessing algorithm of HoD, the distance from $u$ to $w$ should be preserved in the reduced graph, when all nodes not in $S_{i+1}$ are removed. This indicates that $u$ should have a shortcut to $w$, and the shortcut should have a length $\d(u, w)$. Therefore, when HoD performs the forward search from $u$, it can correctly identify the distance from $u$ to $w$. Meanwhile, by the induction hypothesis, HoD can also derive the correct distance from $w$ to $v$. Therefore, the distance from $u$ to $v$ can be correctly calculated by HoD. In a similar manner, we can also show that HoD can return the correct distance from any other node $v \in S_{i+1}$ to $u$, which completes the proof.
%Since $\kappa(v) \ne +\infty$, HoD must have traversed a path $P$ from $s$ to $v$, such that $l(P) = \kappa(v)$. This indicates that $\d(s, v) \le \kappa(v)$. To prove the lemma, it suffices to show that $\d(s, v) \ge \kappa(v)$ also holds.
%
%Assume to the contrary that there exists a path $P'$ in the original graph $G$, such that $l(P') < \kappa(v)$. Without loss of generality, assume that $P' = \langle v_1, v_2, \ldots, v_k\angle$, where $v_1 = s$ and $v_k = v$. %Suppose that we remove from $P'$ any node $v_i$ ($i \in [1, j]$) that has a smaller rank than some node $v_a$ ($a < i$) preceding it. Let $S = \langle v'_1, v'_2, \ldots v'_b \rangle$ be the sequence of nodes remaining on $P_1$. We have $v'_1 = v_1$, since no node precedes $v_1$. In addition, $v'_b = v_j$, since (i)
\end{proof}

\subsection{Space and Time Complexities} \label{sec:p2p-complex}

Overall, the PPD query algorithm of HoD requires $O(n + m_c)$ main memory, where $n$ is the number of nodes in $G$ and $m_c$ is the number of edges in the core graph $\GC$. This is because, during the core search, the algorithm reads $\GC$ into the memory, and it needs to maintain two hash tables and two min-heaps, each of which takes $O(n)$ space.

When processing a query, HoD inserts each node into each min-heap at most once, and it visits each edge in $\GC$, $\GF$, and $\GB$ no more than once. Therefore, the time complexity of the query algorithm is $O(n \log n + m')$, where $m'$ is the total number of edges in $\GC$, $\GF$, and $\GB$. In practice, the query time of HoD tends to be much smaller than this worst-case bound, since the forward and backward searches of HoD usually visit only a small portion of the augmented graph, as illustrated in Section~\ref{sec:overview-query}. The I/O costs of the query algorithm is $O((n + m')/B)$, because HoD scans $\GC$, $\GF$, and $\GB$ exactly once.

%\subsection{Reversed Search} \label{sec:sssp-reversed}
%
%Given the hash table $H$ obtained from the core search, the reversed search of HoD is performed as a sequential scan of the reversed graph $\GR$, where the nodes' adjacency list is stored in descending order their ranks. For each node $v$ visited, HoD checks each edge $e = \langle u, v\rangle$ adjacent to $v$ (recall that $\GR$ contains only incoming edges). If $\kappa(u) \ne +\infty$ and $\kappa(u) + l(e) < \kappa(v)$, then HoD sets $\kappa(v) = \kappa(u) + l(e)$. Once all nodes in $\GR$ are scanned, HoD terminates the reversed search and, for each node $v$, returns $\kappa(v)$ as the distance from $s$ to $v$.


%\section{Shortest Path Queries} \label{sec:path}
%
%Talk about how to store path information for reconstruction.

%\section{Extensions}\label{sec:exten}
%In this section we present two major optimizations for the basic algorithm presented in section ~\ref{sec:details}. The first optimization is called \emph{Node Extension} which more accurately selects transit nodes from the set of local shortest paths in $SelectTransitNode$. The second one is an alternative way of adding shortcuts which greatly improve the query efficiency.
%
%\subsection{Node extension}
%In $SelectTransitNode$, we select the transit nodes to $V_i$ by $V_{i-1}$ and $E_{i-1}$. We examine each local shortest path $p\in\mathcal{P}$ to find an edge $e$ that intersects the inner shell. If $e$ is a shortcut, we need to expand $e$ to find the real transit edge contracted by $e$. However, this expansion would probably upgrade a node which is not previously in $V_{i-1}$. As shown in Figure ~\ref{fig:realedge}, $(u',v')$ is the real-edge and is put into $TE_i$. In this case either $u'$ or $v'$ would be selected into $V_i$, but $u'$ or $v'$ is not necessarily in $V_{i-1}$. As a matter of fact, $(u,v)$ could also be considered a transit edge if all the local shortest paths in $\mathcal{P}$ which passes $(u',v')$ also passes $(u,v)$. When we say a path passes a shortcut we mean that the path passes the shortest path contracted by the shortcut. For example, as shown in Figure ~\ref{fig:level2}, when computing $V_2$, we already have four local shortest paths in $\mathcal{P}$: $p_1$ from $v_1$ to $v_3$, $p_2$ from $v_1$ to $v_4$, $p_3$ from $v_2$ to $v_3$ and $p_4$ from $v_2$ to $v_4$. As for $p_3$, the shortcut $(v_9,v_{10})$ contains a real-edge $(v_6,v_{10})$. Since in $\mathcal{P}$ all the shortest path which passes $(v_6,v_{10})$ also passes $(v_9,v_{10})$ (the sub-path $(v_9,v_6,v_{10})$), in this case it is reasonable to take $(v_9,v_{10})$ as an transit edge instead of $(v_6,v_{10})$.
%
%In addition, here we perform a node extension. We consider not only the real-edge $(u',v')$, but a sub-path extended from $u'$ and $v'$. Let $p=(s,\ldots,u,v,\ldots,t)\in\mathcal{P}$ be a local shortest path found by $FindLocalShortestPath$, then $p$ is a path composed of the nodes in $V_{i-1}$, except that neither of its source $s$ nor target $t$ is necessarily in $V_{i-1}$. Let $(u,v)$ be the edge on $p$ that intersects the inner shell of a cell that contains $s$. We further use $(u',v')$ to denote the real-edge contracted by $(u,v)$. If $(u,v)$ is an original edge in $G$, then let $(u',v')=(u,v)$. We extend the sub-path $(u',v')$ on $p$ by $\alpha$ hops ($\alpha$ is a pre-defined parameter), and we call it \emph{$\alpha$-hops extended path from $(u',v')$ of $p$}. For example, if we set $\alpha=2$, we extend the sub-path $(u',v')$ to $(u_1,u,u',v',v,v_1)$, where $u_1$ is the parent of $u$ (on $p$) and $v_1$ likewise. Note that $(u_1,u,v,v_1)$ is a sub-path on $p$, and $(u',v')$ is contracted  by $(u,v)$.  Let $\mathcal{P}_{(u',v')}\subseteq\mathcal{P}$ be the set of local shortest paths that has $(u',v')$ as its real-edge, and the sub-path $p'=(x,\ldots,y)$ be the longest common sub-path among all the $\alpha$-hops extended path from $(u',v')$ on each $p\in\mathcal{P}_{(u',v')}$. Then we put $(x,y)$ as an imaginary transit edge into $TE_i$ although $x$ and $y$ are not really connected by an original edge or shortcut. Further, either $x$ or $y$ would be selected from $TE_i$ as an transit node into $V_i$. In our experiments we select $\alpha=3$, namely, starting from the real-edge $(u',v')$, we trace three hops backward ($u,u_1,u_2$) and tree forward($v,v_1,v_2$). Because we found that the local shortest paths that share the same real-edge would usually diverge at the third hop.
%
%The key point of why Node-extension optimizes the method is that, we chose a longer common sub-path $(x,y)$ shared by a number of local shortest paths instead of the real-edge $(u',v')$ as the candidates of transit edges, which in turns makes the estimation of the node importance more accurate and plausible. This is consistent with our real-life experience. For example, if a path $p'$ is the common sub-path shared by a number of shortest-paths, when planing a route, we would usually pay more attention at the endpoints of $p'$ instead of the middle points. Observe that in this optimization we only substitute the real-edge with a longest common sub-path as a candidate transit edge for selecting transit node. This substitution would not vary the number of transit nodes since the real-edge and the common sub-path cover the same number of local shortest paths.
%
%\subsection{Query indexing}
%The second optimization is that, we use an alternative way of adding shortcuts instead of the one described in subsection ~\ref{label{sub:shortcuts}}. After we obtain a partition of nodes into levels $\mathcal{L}=\{L_0,L_1,\ldots,L_h\}$, we impose a total order on the nodes: The nodes in $L_{i+1}$ has a higher rank than those in $L_i$, and within the same level, the node covers more local shortest paths has a higher rank. Now we remove all the shortcuts added before and reconstruct the index in this way: we add two types of shortcuts: \emph{Jumping shortcuts} and \emph{Query shortcuts}. To accelerate the construction of jumping shortcuts, we also add a third type of shortcut \emph{level shortcuts}. Actually not all the level shortcuts are used in the query, hence, after constructing jumping shortcuts, we only preserve a subset of level shortcuts which are useful in the queries, and we call them query shortcuts.
%
%\subsubsection{Jumping shortcuts and query shortcuts}
%Before constructing the shortcuts, we slightly adjust the nodes layers. We define $\mathcal{R}=\{R_0,\ldots,R_h\}$, where $R_i=\bigcup\limits_{j=i}^h{R_j}$ for $0\leq i\leq h$, i.e. $R_i$ is the set of nodes that are at least in level $i$. We start from $i=1$ and $E_0=E$. At the $i$th iteration, firstly we impose a grid on $G$. The grid scale is the same as the one imposed before when computing the node levels, i.e. $g_i\times g_i$. For each $v\in R_i$, we use a similar algorithm to compute the layer-i neighbours of $v$ as described in \ref{sub:shortcuts}. For $v\in R_i$, the layer-i neighbours of $v$ refer to those nodes: if for any node $w$ such that $SP(v,w)$ passes at least one node in $R_i$, and $u$ on $SP(v,w)$ is a node in $R_i$ that is closet to $v$, then $u$ is the layer-i neighbour of $v$. The set of edges (or shortcuts) that connect each $v\in R_i$ to its layer-i neighbours is represented as $E_i$, and we call the edges in $E_i$ level shortcuts. Then at the $i+1$th iteration, the computation of the layer-(i+1) neighbours of a node $v\in R_{i+1}$ can reuse the edges in $E_i$ as shown in Figure ~\ref{fig:levelshortcuts}. The level shortcuts in $E_i$ guarantee the connectivity because $V_{i+1}\subseteq V_i$. %For a node $v\in V_{i+1}$, we perform a Dijkstra traversal from $v$, meanwhile we maintain a counter $ufb$ to count the unfinished branches as described in algorithm ~\ref{alg:addshortcuts}. Different from algorithm ~\ref{alg:addshortcuts}, during the traversal, we only visit the nodes in $V_i$. The level shortcuts in $E_i$ guarantee the connectivity because $V_{i+1}\subseteq V_i$.
%
%%\begin{figure}
%%\centering
%%\includegraphics[width = 3in]{figures/levelshortcuts.eps}
%%\caption{Level shortcuts} \label{fig:levelshortcuts}
%%\end{figure}
%
%\begin{figure}[t]
%%\begin{small}
%\begin{minipage}[t]{1.63 in}
%\centering
%\includegraphics[width = 1.67in]{figures/levelshortcuts.eps}
%\vspace{-3.49mm}
%\figcapup \caption{Level shortcuts $\quad$} \label{fig:levelshortcuts} \figcapdown
%\end{minipage}
%\begin{minipage}[t]{1.85 in}
%\centering
%%\hspace{3mm}
%\includegraphics[width = 1.67in]{figures/jumpingshortcut.eps}
%\figcapup \caption{Jumping shortcuts $\quad$} \label{fig:jumpingshortcut} \figcapdown
%\end{minipage}
%%\end{small}
%\end{figure}
%
%With the level shortcuts we can construct the jumping shortcuts in this way. Starting with $i=1$, at the $i$th iteration, we impose a grid on $G$ sized of $g_i\times g_i$. For each $s\in V-R_i$, (ATTENTION: or $s\in V-R_{i+1}$??) we add a shortcut to its transit node in $R_i$. Let $C$ be the cell that contains $s$. We consider a sub-graph that overlaps with the outer shell of $C$. Then we build a Dijkstra spanning tree rooted from $s$. During the Dijkstra traversal we only visit the nodes in $R_{i-1}$ connected by the level shortcuts. Then from a leaf node $t$, backtrack the path to its root $s$. Let $u$ on the path be the node in $R_i$ that is closet to $v$, then we add a shortcut from $s$ to $u$, which is called jumping shortcut. Such $u$ exists because the leaf node $t$ is outside the outer shell of $C$, and by definition the local shortest path from $s$ to $t$ would pass a transit node, which would be at least in $L_i$ or even higher level. In a word, a jumping shortcut connects a node to the transit node of its cell as illustrated in Figure ~\ref{fig:jumpshortcuts}.
%
%%\begin{figure}
%%\centering
%%\includegraphics[width = 3in]{figures/jumpingshortcut.eps}
%%\caption{Jumping shortcuts} \label{fig:jumpingshortcut}
%%\end{figure}
%
%The query shortcuts preserve a subset of the level shortcuts. For each $v\in R_i$, previously we add a level shortcut from $v$ to its layer-i neighbour $u$.  Now we preserve the shortcut only if $Rank_v<Rank_u$.
%
%Although we present the construction of level shortcuts and jumping shortcuts in two separate processes, these two constructions could be performed at the same time, i.e. at the $i$th iteration, we add level shortcuts that connect the nodes in $R_i$, and jumping shortcuts to the nodes in $R_i$ by the level shortcuts added in the $i-1$th iteration.
%
%\subsubsection{Query method}
%Now the query method works in the following way: for a given source $s$ and target $t$, we instantiate two Dijkstra traversal respectively from $s$ and $t$. During the traversal we use two priority queues $Q_f$ and $Q_b$ which respectively maintain the forward search from $s$ and the backward search from $t$. Initially $Q_f$ (resp. $Q_b$) contains $s$ (resp. $t$) only. Then we compute how far it is between $s$ and $t$. Based on the geometrical location of $s$ and $t$, we compute the highest level $l$, such that in the $g_l\times g_l$ scale cell, $t$ is beyond the outer shell of the cell that contains $s$, and in the $g_{l+1}\times g_{l+1}$ level scale, $t$ is inside the outer shell. If $l$ is greater than $l_s$, where $l_s$ is the level of $s$, then we dequeue $s$ and enqueue the transit nodes of $s$ into $Q_f$ by jumping shortcuts at level $l$. As illustrated in Figure ~\ref{fig:jumpingshortcut}, we first reach the transit nodes of $s$ (at level $l$) by jumping shortcuts, because the jumping shortcuts direct the search to the nodes that are highly probable on the right shortest path. After that we can perform a similar bidirectional Dijkstra search as described in section ~\ref{sub:query}. If the level of $s$ is greater than $l$, such that from $s$ there is no jumping shortcut at level $l$, then we can start the Dijkstra traversal from $s$. Since the search would only visit a node with higher rank, and $s$ itself is a node of higher rank, so the search would quickly converge to the node with highest rank in the path.
%
%\subsection{Directed graphs}\label{subsec:directedgraphs}


==> 8-Conclusions/Conclusions.tex <==
\section{Conclusions}\label{sec:conclu}

%This paper presents {\em HoD}, a practically efficient index structure for distance queries on disk-resident large graphs. In particular, HoD supports both directed and undirected graphs, and it efficiently handles {\em single source distance (SSD) queries} and {\em point-to-point distance (PPD) queries}. This contrasts the existing methods, which (i) are applicable only on undirected graphs and (ii) do not optimize the efficiency of PPD queries. With extensive experiments on a variety of large graphs, we demonstrate that HoD significantly outperforms the state of the art in terms of query efficiency, space consumption, and pre-computation costs. For future work, we plan to investigate how HoD can be extended to handle dynamic graphs that change with time.

This paper presents HoD, a practically efficient index structure for distance queries on massive disk-resident graphs. In particular, HoD supports both directed and undirected graphs, and it efficiently handles {\em single-source shortest path (SSSP) queries} and {\em single-source distance (SSD) queries} under memory-constrained environments. This contrasts the existing methods, which either (i) require that the dataset fits in the main memory during pre-computation and/or query processing, or (ii) support only undirected graphs. With extensive experiments on a variety of real-world graphs, we demonstrate that HoD significantly outperforms the state of the art in terms of query efficiency, space consumption, and pre-computation costs. For future work, we plan to investigate how HoD can be extended to (i) support point-to-point shortest path and distance queries and (ii) handle dynamic graphs that change with time.



%Some bullshit conclusion and future work.
\balance

